A Moment in the Sun: Solar Nowcasting from Multispectral Satellite Data using Self-Supervised Learning

Solar energy is now the cheapest form of electricity in history. Unfortunately, significantly increasing the grid's fraction of solar energy remains challenging due to its variability, which makes balancing electricity's supply and demand more difficult. While thermal generators' ramp rate -- the maximum rate that they can change their output -- is finite, solar's ramp rate is essentially infinite. Thus, accurate near-term solar forecasting, or nowcasting, is important to provide advance warning to adjust thermal generator output in response to solar variations to ensure a balanced supply and demand. To address the problem, this paper develops a general model for solar nowcasting from abundant and readily available multispectral satellite data using self-supervised learning. Specifically, we develop deep auto-regressive models using convolutional neural networks (CNN) and long short-term memory networks (LSTM) that are globally trained across multiple locations to predict raw future observations of the spatio-temporal data collected by the recently launched GOES-R series of satellites. Our model estimates a location's future solar irradiance based on satellite observations, which we feed to a regression model trained on smaller site-specific solar data to provide near-term solar photovoltaic (PV) forecasts that account for site-specific characteristics. We evaluate our approach for different coverage areas and forecast horizons across 25 solar sites and show that our approach yields errors close to that of a model using ground-truth observations.

==> model.tex <==
In this section, we describe our complete methodology for solar forecasting.
We first describe our neural network model for self-supervised learning on raw satellite observations.
Then, we describe a simple auto-regressive model for solar generation forecasting that can leverage forecasts from the self-supervised model.

\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.95\columnwidth]{graphs/graphs/design}}
\vspace{-0.3cm}
\caption{\emph{Overview of our complete solar forecasting approach.}}
% \vspace{-0.5cm}
\label{design}
\end{center}
\vspace{-0.5cm}
\end{figure}

\subsection{Self-supervised modeling of satellite data}
Short-term forecasting of solar power needs to take into account the recent changes to solar irradiation at the surface and how it will evolve in a short span of time. 
% This is different from traditional forecasting methods which is usually hours ahead in the future and needs to model complex, long-term relationships between atmospheric phenomenon, for example using numerical weather models. 
For example, cloud cover and movement is a key component that determines the amount of down-welling solar irradiation. Indeed, one of the prominent approach to solar modeling and forecasting is through using coarse measurements of cloud cover, called Okta \cite{okta-mirror,dong}. This is also the major source of error in current models as these measurements are coarse and imprecise \cite{dong,buildsys,dsr2020}.
\citet{buildsys} instead showed that GOES visible bands are highly correlated with solar irradiance at the surface, allowing accurate inference of solar power through machine learning models trained on historic generation data with GOES visible bands as inputs.

We seek to utilize this relationship (Fig.~\ref{solarchannel}) for forecasting by using deep neural networks to implicitly model the short-term changes in the values of the visible bands of GOES.
We will use this model to forecast future values of the visible channels which in turn will help in predicting solar generation, owing to this relationship between channel and solar generation.
Figure \ref{design} shows an overview of our modeling approach.
Given a set of solar sites of interest, we consider an area of $w\times h$ around the site and extract the 3 visible channels of satellite data from the GOES-16 satellite. We get a temporal sequence of $w\times h$ images over time from the satellite, with the target site always at the center of the image as this is a geo-stationary satellite.
We consider sequence of upto 5 such images at a time with an interval of 15 minutes between images, spanning an hour of satellite imagery prior to the last image. 
Each 3D satellite image is processed through a multi-layer convolutional neural network (CNN) into a fixed $d$-dimensional representation at each time-step.
The sequence of CNN representations from each step are then fed into a long short-term memory network (LSTM) to capture the temporal evolution relevant for predicting observations at future time-steps.

The final step output is from an LSTM, and, after processing 4 sequences of images (1 hour), is passed through a dense layer with sigmoid output units to predict the value of the visible channels at the site location after 15 minutes.
The CNN-LSTM model is trained end-to-end using mean-squared error, with respect to the true future satellite values, as the loss function.
Note that we only train one global model by combining satellite data across multiple sites.
This enables modeling of shared statistical properties rather than overfitting to the peculiar characteristics of an isolated site.
Moreover, this also provides abundant data for learning a useful CNN-LSTM model which typically don't work well with small datasets.



\subsection{Solar generation forecasting}
\label{sec:solar}
Given a trained CNN-LSTM model that can generate future satellite observations at a given site, we aim to leverage these predictions in a model for solar power forecasting at any solar installation site of interest.
\citet{buildsys} showed that the current channel value can be used to infer the site-specific solar generation by training a simple regression model on historic data which helps correlate satellite observations with solar installation specific characteristics.
We build on that finding by considering the following auto-regressive model for forecasting near-term solar output:
\begin{equation}
    P_{t+1} = f(P_t, C_{t+1}, T_{t}) \label{eq:solar_model}
\end{equation}
where $P_t$ is the solar power generated, $C_t$ are the satellite visible channel values and $T_t$ is the temperature at time $t$. $f(\cdot)$ is a regression model, such as support vector regression, that models the relationship between the input and output variables using historical data.
Temperature is an important component of solar generation as solar panel efficiency is sensitive to the surrounding temperature \cite{dong}.
Note that we use $C_{t+1}$ instead of $C_t$ in \eqref{eq:solar_model}. A major component of change in $P_{t+1}$ from $P_{t}$ is captured in the change in $C_{t+1}$ from $C_{t}$. This complex relationship is modeled using our CNN-LSTM model, described above, which allows us to predict $\hat{C}_{t+1}$, an estimate of true channel values at $t+1$ to use in the auto-regressive model in \eqref{eq:solar_model}.

